Fast Entropy-Based Methods of Word-Level Confidence Estimation for End-To-End Automatic Speech Recognition

This paper presents a class of new fast non-trainable entropy-based confidence estimation methods for automatic speech recognition. We show how per-frame entropy values can be normalized and aggregated to obtain a confidence measure per unit and per word for Connectionist Temporal Classification (CTC) and Recurrent Neural Network Transducer (RNN-T) models. Proposed methods have similar computational complexity to the traditional method based on the maximum per-frame probability, but they are more adjustable, have a wider effective threshold range, and better push apart the confidence distributions of correct and incorrect words. We evaluate the proposed confidence measures on LibriSpeech test sets, and show that they are up to 2 and 4 times better than confidence estimation based on the maximum per-frame probability at detecting incorrect words for Conformer-CTC and Conformer-RNN-T models, respectively.

==> bar_chart_ctc.tex <==
% Define bar chart colors
%
\definecolor{bblue}{HTML}{4F81BD}
\definecolor{rred}{HTML}{C0504D}
\definecolor{ggreen}{HTML}{9BBB59}
\definecolor{ppurple}{HTML}{9F4C7C}

\begin{figure}[ht]
\begin{tikzpicture}
    % \renewcommand\baselinestretch{1.5}
    \begin{axis}[
        title=CTC,
        title style={at={(0.5,0.97)}},
        width  = \linewidth,
        height = 6cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        ymax=90,
        bar width=10pt,
        ymajorgrids = true,
        ylabel = {$\mathrm{AUC}_\mathrm{NT}$, $\%$},
        symbolic x coords={\textit{test-other},\textit{test-other-snr\_30},\textit{test-other-snr\_0}},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.15,
        ymin=0,
        % nodes near coords,  
        nodes near coords align={vertical},  
        legend cell align=left,
        legend style={
            at={(0.2,1.0)},
            anchor=north
            % legend columns=2
        },
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
            coordinates {(\textit{test-other}, 32.41) (\textit{test-other-snr\_30},35.17) (\textit{test-other-snr\_0},81.50)};

        \addplot[style={rred,fill=rred,mark=none}]
             coordinates {(\textit{test-other},37.46) (\textit{test-other-snr\_30},40.76) (\textit{test-other-snr\_0},83.36)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(\textit{test-other},45.18) (\textit{test-other-snr\_30},48.35) (\textit{test-other-snr\_0},78.11)};

        \addplot[style={ppurple,fill=ppurple,mark=none}]
             coordinates {(\textit{test-other},47.01) (\textit{test-other-snr\_30},50.29) (\textit{test-other-snr\_0},82.65)};

        \legend{$\prod_{p}F_{max}(p)$,$\prod_{p}F_{eg}(p)$,$\operatorname*{mean}_{p}F_{ets}(p)$,$\min_{p}F_{ets}(p)$}
    \end{axis}
\end{tikzpicture}
\vspace{-10pt} % adjust this
\caption{$\mathrm{AUC}_\mathrm{NT}$ in $\%$ for CTC and different noise conditions.}
\label{fig:bar-ctc}
\end{figure}


==> bar_chart_rnnt.tex <==
% Define bar chart colors
%
\definecolor{bblue}{HTML}{4F81BD}
\definecolor{rred}{HTML}{C0504D}
\definecolor{ggreen}{HTML}{9BBB59}
\definecolor{ppurple}{HTML}{9F4C7C}

\begin{figure}[ht]
\begin{tikzpicture}
    % \renewcommand\baselinestretch{1.5}
    \begin{axis}[
        title=RNNT,
        title style={at={(0.5,0.97)}},
        width  = \linewidth,
        height = 6cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        ymax=90,
        bar width=10pt,
        ymajorgrids = true,
        ylabel = {$\mathrm{AUC}_\mathrm{NT}$, $\%$},
        symbolic x coords={\textit{test-other},\textit{test-other-snr\_30},\textit{test-other-snr\_0}},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.15,
        ymin=0,
        % nodes near coords,  
        nodes near coords align={vertical},  
        legend cell align=left,
        legend style={
            at={(0.2,1.0)},
            anchor=north
            % legend columns=2
        },
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
            coordinates {(\textit{test-other}, 21.28) (\textit{test-other-snr\_30},22.34) (\textit{test-other-snr\_0},62.33)};

        \addplot[style={rred,fill=rred,mark=none}]
             coordinates {(\textit{test-other},27.70) (\textit{test-other-snr\_30},28.93) (\textit{test-other-snr\_0},68.92)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(\textit{test-other},32.61) (\textit{test-other-snr\_30},36.55) (\textit{test-other-snr\_0},70.49)};

        \addplot[style={ppurple,fill=ppurple,mark=none}]
             coordinates {(\textit{test-other},47.17) (\textit{test-other-snr\_30},49.91) (\textit{test-other-snr\_0},77.63)};

        \legend{$\prod_{p}F_{max}(p)$,$\prod_{p}F_{eg}(p)$,$\operatorname*{mean}_{p}F_{ets}(p)$,$\min_{p}F_{ets}(p)$}
    \end{axis}
\end{tikzpicture}
\vspace{-10pt} % adjust this
\caption{$\mathrm{AUC}_\mathrm{NT}$ in $\%$ for RNNT and different noise conditions.}
\label{fig:bar-rnnt}
\end{figure}

